PINSAT: Parallelized Interleaving of Graph Search and Trajectory Optimization for Kinodynamic Motion Planning

Trajectory optimization is a widely used technique in robot motion planning for letting the dynamics and constraints on the system shape and synthesize complex behaviors. Several previous works have shown its benefits in high-dimensional continuous state spaces and under differential constraints. However, long time horizons and planning around obstacles in non-convex spaces pose challenges in guaranteeing convergence or finding optimal solutions. As a result, discrete graph search planners and sampling-based planers are preferred when facing obstacle-cluttered environments. A recently developed algorithm called INSAT effectively combines graph search in the low-dimensional subspace and trajectory optimization in the full-dimensional space for global kinodynamic planning over long horizons. Although INSAT successfully reasoned about and solved complex planning problems, the numerous expensive calls to an optimizer resulted in large planning times, thereby limiting its practical use. Inspired by the recent work on edge-based parallel graph search, we present PINSAT, which introduces systematic parallelization in INSAT to achieve lower planning times and higher success rates, while maintaining significantly lower costs over relevant baselines. We demonstrate PINSAT by evaluating it on 6 DoF kinodynamic manipulation planning with obstacles.

==> 06bsplineopt.tex <==
\pdfoutput=1

% This section explains the operation we perform to lift the low-D edges $e\in\Edges$ in the graph $G$ to full-D. Specifically, given an edge, we describe our trajectory optimization setup to incorporate the cost and constraints in $\statespace$ in addition to those imposed by the edge living in $\lowdspace$. 

This section solely explains the abstract optimization over the length and duration of B-splines that satisfy the obstacle, duration, derivative, and boundary constraints. In the next section, we describe how it is utilized within \epase's parallel graph search. 

% In this section, we will describe how we formulate and utilize trajectory optimization to lift the edges in the low-D graph to full-D space. For applications with fully actuated systems that do not involve transporting heavy payloads, or making and breaking contacts with the environment, near-dynamic feasibility can be achieved by parameterizing trajectories with polynomials and splines [cite]. In this work, we use a rich class of parametric splines with very high interactivity and local control called B-splines. There is a recent interest in using B-splines for trajectory generation in manipulation due to their geometric properties that allow representing joint position and velocity constraints as linear constraints on polynomial bases [cite].  We will first provide background on the recursive B-spline representation, and then present our trajectory optimization formulation for generating these B-splines under kinematic constraints. Following this, we will explain how we utilize the trajectory generator in two different ways in PINSAT. 

\subsection{Decoupling Optimization over Trajectory and its Duration}
It is easy to observe from Eq. \ref{eq:obj} that there is a coupling between the trajectory $\traj(t)$ and its duration $T$. For simultaneous optimization over the $\traj$ and $T$, we decouple them by introducing a trajectory coordinate $u \in [0, 1]$ and a mapping to convert this coordinate to the actual time, $t=\timemap(u)$ [cite]. Let the mapping $\timemap$ be monotonously increasing with $\timemap(0) = 0$ and $\timemap(1)=T$ and $\traj(t) = \traj(\alpha(u)) = \utraj(u)$. With this transformation, the derivatives of the trajectory can be derived as
\begin{equation}
    \trajdot(t) = \frac{d\traj(\alpha(u))}{d\alpha}\frac{d\alpha(u)}{du}\frac{du}{dt} = \frac{d\utraj(u)}{du}\frac{du}{dt}
    \label{eq:trajderiv}
\end{equation}
Dropping the arguments for simplicity
\begin{multline*}
    \trajddot(t) = \frac{d}{dt}\left(\frac{d\traj}{d\alpha}\right) \frac{d\alpha}{du}\frac{du}{dt} \\ + \frac{d\traj}{d\alpha}\frac{d}{dt}\left(\frac{d\alpha}{du}\right)\frac{du}{dt} + \cancelto{0}{\frac{d\traj}{d\alpha}\frac{d\alpha}{du}\frac{d}{dt}\left(\frac{du}{dt}\right)}
\end{multline*}
\begin{multline}
    \trajddot(t) = \frac{d^2\traj}{du^2}\left(\frac{du}{dt}\right)^2 + \frac{d\traj}{d\alpha}\frac{d}{dt}\left(\frac{d\alpha}{du}\right)\frac{du}{dt} \\ = \frac{d\utraj^2}{du^2}\left(\frac{du}{dt}\right)^2 + \frac{d\utraj}{ds}\frac{d^2u}{dt^2}
    \label{eq:trajdderiv}
\end{multline}
Similarly
\begin{equation}
    \trajdddot(t) = \frac{d^3\utraj}{du^3}\left(\frac{du}{dt}\right)^3 + 3\frac{d^2\utraj}{du^2}\frac{d^2u}{dt^2}\frac{du}{dt} + \frac{d\utraj}{du}\frac{d^3u}{dt^3}    
    \label{eq:trajddderiv}
\end{equation}

\subsection{Transcription for Optimizing B-splines} Now we can apply the decoupling introduced above to the optimization in Eq. \ref{eq:obj} with the new trajectory coordinate $u$ and the map $\utraj$ introduced above. The derivative of the B-spline curve $\traj^{(j)}(t)$ in terms of the derivative of the B-spline basis $N_{i, k}^{(j)}(t)$ is given in Eq. \ref{eqn:bsderiv1}. Using this relation the derivative of the B-spline curve with the trajectory coordinate $\utraj^{(j)}(u)$ in terms of the derivative's control points $\textbf{p}_i^{(j)}$ can be derived as [cite]
\begin{equation}
    \utraj^{(j)}(u) = \sum_{i=0}^{n-j} \textbf{p}_i^{(j)} N_{i, k-j}(u)
    \label{eq:bsdervi2}
\end{equation}
where $\textbf{p}_i^{(j)}$ is given as
\begin{equation}
\textbf{p}_i^{(j)}= \begin{cases}\textbf{p}_i & j=0 \\ \frac{k-j+1}{u_{i+k+1}-u_{i+j}}(\textbf{p}_{i+1}^{(j-1)}-\textbf{p}_i^{(j-1)}) & j>0\end{cases}
\end{equation}


% In this work, we use the relation $t = \alpha(u) = T*u$ between time and the trajectory coordinate. Under this relation, we can see that
% \begin{align}
%     \frac{du}{dt} = \frac{1}{T} \quad \text{and} \quad \frac{d^2u}{dt^2} = 0
% \end{align}
In this work, we use $t = \alpha(u) = Tu$. So $\frac{du}{dt} = \frac{1}{T}$ and $\frac{d^2u}{dt^2} = \frac{d^3u}{dt^3} = 0$ and Eq. \ref{eq:trajderiv} - Eq. \ref{eq:trajddderiv} becomes 
\begin{align}
    % \trajdot(t) = \frac{1}{T}\frac{d\utraj}{du} \quad \trajddot(t) = \frac{1}{T^2}\frac{d^2\utraj}{du^2} \quad \trajdddot(t) = \frac{1}{T^3}\frac{d^3\utraj}{du^3}
    \traj^{(j)}(t) = \frac{1}{T^j}\frac{d^j\utraj}{du^j} \quad \text{where} \ j=\{1,2,3\}
    \label{eq:ttou}
\end{align}

The optimization in Eq. \ref{eq:obj} can be transcribed into a parameter optimization problem over the control points of the B-spline trajectory $\textbf{P} = \{\textbf{p}_0, \ldots, \textbf{p}_m\}$ and the duration of the trajectory $T$ using Eq. \ref{eq:ttou} as
\begin{subequations}
\begin{alignat}{2}
% & \traj_{\state^S\state^G}(t), T_{\state^S\state^G} = \argmin_{\traj(t), T}\quad w_1T + w_2\int_0^T \traj(t)dt \\ 
\min_{\textbf{p}_0, \ldots, \textbf{p}_m, T} \quad & w_1T + w_2\sum_{i=0}^{m-1} \norm{\textbf{p}_{i+1} - \textbf{p}_i}_2 \label{eq:uobj1}\\ 
\textrm{s.t.} \quad & t_{\text{min}} \leq T \leq t_{\text{max}} \label{eq:uobj2}\\
& \textbf{p}_0 = \state^S,  \textbf{p}_m = \state^G \in \goalreg \label{eq:uobj3}\\
& |\textbf{p}_i^{(j)}| \preceq T^j\traj^{(j)}_{\text{lim}}; i=\{0,\ldots,m\}, j=\{1,2,3\} \label{eq:uobj4}\\
% & \utraj_{\textbf{p}_i}(u) \in \freespace; u\in[0,1], i=\{0,\ldots,m\} \label{eq:uobj5}\\
% & \utraj_{\textbf{p}_i}(u) \in \mathcal{C}^\gamma(\mathbb{R}); u\in[0,1], i=\{0,\ldots,m\} \label{eq:uobj6}
& \utraj_{\textbf{P}}(u) \in \freespace; u\in[0,1] \label{eq:uobj5}
% & \utraj_{\textbf{P}}(u) \in \mathcal{C}^\gamma(\mathbb{R}); u\in[0,1]\label{eq:uobj6}
\end{alignat}
\label{eq:uobj}
\end{subequations}
where $\utraj_{\textbf{P}}$ is the trajectory reconstructed using the control points $\textbf{P}$ (Eq. \ref{eq:ctrlvec}). From the properties of B-splines [cite], we know that the B-spline curve is entirely contained inside the convex hull of its control points. We leverage this property to formulate Eq. \ref{eq:uobj1} and Eq. \ref{eq:uobj4}. So it is enough to just enforce the trajectory derivative constraints at the control points (Eq. \ref{eq:uobj4}) instead of checking if the curve satisfies them for all $u$ (and therefore for all $t$). 
\begin{remark}
The constraint on the control points in Eq. \ref{eq:uobj4} is a sufficient but not necessary condition to enforce the limits on derivatives. In other words, it is possible to have control points outside the limits $\pm T^j\traj^{(j)}_{\text{lim}}$ and still have the curve satisfy these limits.
\label{rem:suff}
\end{remark}

\subsection{B-spline Trajectory Reconstruction} Once the control point vector $\textbf{P}$ and the duration of trajectory $T$ are found by solving Eq. \ref{eq:uobj}, the trajectory and its derivatives can be computed given the choice of B-spline basis $N_{i, k}(t)$ (Eq. \ref{eq:bsb}) and the knot vector $\textbf{T}$ (Eq. \ref{eq:knotvec}) using Eq. \ref{eq:bs} and Eq. \ref{eq:bsdervi2}. We also use this reconstruction to validate Eq. \ref{eq:uobj5} within every iteration of the solver routine for obstacle avoidance, early termination and constraint satisfaction.


